Anatomizing Deep Learning Inference in Web Browsers

Web applications have increasingly adopted Deep Learning (DL) through in-browser inference, wherein DL inference performs directly within Web browsers. The actual performance of in-browser inference and its impacts on the quality of experience (QoE) remain unexplored, and urgently require new QoE measurements beyond traditional ones, e.g., mainly focusing on page load time. To bridge this gap, we make the first comprehensive performance measurement of in-browser inference to date. Our approach proposes new metrics to measure in-browser inference: responsiveness, smoothness, and inference accuracy. Our extensive analysis involves 9 representative DL models across Web browsers of 50 popular PC devices and 20 mobile devices. The results reveal that in-browser inference exhibits a substantial latency gap, averaging 16.9 times slower on CPU and 4.9 times slower on GPU compared to native inference on PC devices. The gap on mobile CPU and mobile GPU is 15.8 times and 7.8 times, respectively. Furthermore, we identify contributing factors to such latency gap, including underutilized hardware instruction sets, inherent overhead in the runtime environment, resource contention within the browser, and inefficiencies in software libraries and GPU abstractions. Additionally, in-browser inference imposes significant memory demands, at times exceeding 334.6 times the size of the DL models themselves, partly attributable to suboptimal memory management. We also observe that in-browser inference leads to a significant 67.2% increase in the time it takes for GUI components to render within Web browsers, significantly affecting the overall user QoE of Web applications reliant on this technology

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> tex/availability.tex <==
\section*{Data Availability}
We provide all of the code and documents in the supplementary material. We will open-source them on paper acceptance.

==> tex/discussion.tex <==
\revise{
\section{Discussion}

\textbf{Impact at large scale.} This paper highlights that there remains a notable performance gap between in-browser inference and native inference, indicating the need for performance enhancement in in-browser inference. For instance, completing the set of SIMD instructions missing in Wasm could speed up in-browser inference. This enhancement would not only benefit in-browser inference but would also aid other applications utilizing Wasm~\cite{wasm-simd-v8, wasm-use-case}. 

Additionally, in developing large-scale Web services, it is crucial for developers to take into consideration the extensive range of device capacities. This diverse spectrum of device capabilities necessitates a thoughtful approach to design, ensuring that services are affordable and efficient across all types of hardware. Specifically, it is advisable to leverage discrete GPUs for inference tasks to capitalize on their superior processing power and speed whenever they are available. This strategy can significantly boost performance and QoE by accelerating data processing tasks. However, when discrete GPUs are not available, developers should strategically segregate rendering and inference tasks. By allocating these processes to different hardware components, Web applications can optimize resource usage and prevent resource competition, helping enhance the overall QoE. 

Moreover, developers can enhance service adaptability by selecting different models based on the performance characteristics of GPUs and CPUs. This can be effectively managed through hardware profiling of GPUs or by establishing performance benchmarks on CPUs. Such an approach allows for the dynamic selection of computational models that best fit the hardware's capabilities.

\noindent\textbf{Future work.} Optimizing in-browser inference performance is a crucial issue. Our analysis has already indicated that on the CPU side, the main challenges during the prediction stage of in-browser inference stem from environmental differences between native and browser settings. Future work could focus on addressing these issues. For instance, expanding the SIMD instruction set in Wasm to support more efficient operations, such as FMA, could enhance performance significantly. Another potential approach could be to bypass Wasm altogether and implement model kernels, such as matrix multiplication, directly within the browser's JavaScript engine. Since browsers can directly access advanced hardware features and bypass the Wasm interpreter, this could substantially improve inference performance. We are currently exploring optimizations in this direction.
For the warmup phase, considering the high in-browser compilation overhead associated with WebGL, introducing support for importing precompiled intermediate representations into the browser could significantly reduce latency during this stage. This approach would streamline the process, allowing for quicker start-up times and enhancing the overall responsiveness of web applications utilizing in-browser inference. We leave this as a future direction to further optimize the in-browser inference performance.
As for the memory footprint of in-browser inference, we aim to optimize the memory management mechanism of the inference framework. Specifically, this optimization mainly includes the following steps: (1) First, during the model conversion phase, it is necessary to retain the model structure and information about each kernel. (2) Based on this information, obtain the memory access patterns and use optimized memory pool techniques to pre-calculate the strategy of memory management and allocation~\cite{wang2022melon}. (3) Save this information along with the model files so that the inference framework can download and reduce the inference memory footprint.

In summary, our future work primarily focuses on optimizing the performance of in-browser inference, as enhancing inference performance will inevitably lead to improvements in QoE. For instance, lower latency means that devices have more time to process user requests and the DL model can handle more video frames. Additionally, conserving memory footprint will allow browsers to operate more smoothly, avoid stuttering, and thus enhance the smoothness QoE.
}

==> tex/fig-breakdown-latency-distribution.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/tfjs-breakdown-top5op-opLatency-distribution.pdf}
    \caption{Top-5 operators latency distribution.}
    \label{fig:tfjs-breakdown-top5-opLatency-distribution}
\end{figure*}

==> tex/fig-inter-opLatency-distribution.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/inter-opLatency-distribution.pdf}
    \caption{Inter-device kernel latency distribution.}
    \label{fig:inter-opLatency-distribution}
\end{figure}

==> tex/fig-inter-utilization-distribution.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/inter-utilization-distribution.pdf}
    \caption{Inter-device utilization distribution.}
    \label{fig:inter-utilization-distribution}
\end{figure}

==> tex/fig-intra-latency+utilization-distribution.tex <==
\begin{figure*}[t]
    \centering		
	\includegraphics[width=0.8\linewidth]{figures/intra-distribution.pdf}
    \vspace{-3mm}
    \caption{Intra-device latency and utilization distribution. ``M*'' is the model ID and it is the same with Table~\ref{tab:e2e-native-all}}
    \label{fig:intra-latency+utilization-distribution}
\end{figure*}

==> tex/fig-latency-percentage.tex <==
\begin{figure}[t]
	\centering					
	\begin{minipage}[b]{0.2\textwidth}
		\includegraphics[width=1\textwidth]{figures/tfjs-wasm-opLatency-percentage.pdf}
		\subcaption{wasm}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.2\textwidth}
		\includegraphics[width=1\textwidth]{figures/tfjs-webgl-opLatency-percentage.pdf}
		\subcaption{webgl}
	\end{minipage}
\vspace{-5pt}
\caption{The kernel latency percentage of different backend.\shiqi{can describe by text?}}
\label{fig:latency-perecentage}
\end{figure}


==> tex/fig-resnet50-breakdown.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/resnet50-wasm-latency-breakdown.pdf}
    \vspace{-4mm}
    \caption{ResNet50 latency in wasm with different technique enabled. ''-S/-T`` denotes multithreading/SIMD.}
    \label{fig:resnet50-breakdown}
\end{figure}

==> tex/fig-tfjs-wasm-breakdown-e2e-latency.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/tfjs-wasm-breakdown-e2e-latency.pdf}
    \vspace{-3.5mm}
    \caption{Model inference latency. ``-S/T'' means enabling SIMD/multi-threading.}
    \label{fig:wasm-breakdown-e2e-latency}
\end{figure*}

==> tex/fig-top5kernel-latency-distribution.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{figures/tfjs-top5kernel-latency-distribution.pdf}
    \vspace{-5pt}
    \caption{The top5 kernel latency distribution of different backends.}
    \label{fig:top5kernel-latency-distribution}
\end{figure}


==> tex/implication-deprecated.tex <==
\input{tex/tab-qoe-fps}
\section{Implications and Opportunities}
\label{sec:implication}
    
    In this section, we summarize the implications of our findings and propose some opportunities to prompt deploying DL into browser.

    \textbf{For framework developers.} Inspired from \textbf{F1}, \textbf{F2}, \textbf{F4} and \textbf{F5}, latency of different models is rather different, because of different latency patterns of kernels. Existing acceleration techniques contributes unequally to each kernel. For example, wasm is compiled ahead of time, resulting in the compiled kernels to keep the same among different devices. It introduces an opportunity to apply JIT compilation to wasm, so that the compiled binary is most suitable for devices. These findings encourage framework developers to design and optimize each kernel specially.
    The second is memory management, inspired from \textbf{F3}. Memory management is less considered during inference. However, according to our measurement result, memory can be the bottleneck for in-browser inference, which will significantly hinder the potential applications, like online image generation. 
    % Efficient memory management is critical for in-browser scenario.
    It encourages the developers to design and integrate efficient memory management approaches to frameworks.
    The third is acceleration (multi-thread and SIMD), inspired from \textbf{F1}. According to our breakdown analysis, different kernel prefers different acceleration. Take memory-intensive kernels as example, multi-thread may even degrade their performance due to inefficient data sharing mechanism, i.e., through message passing among Web Workers. It is critical to apply different acceleration approach to make kernel run faster. 
    Moreover, two types of available hardware also introduces new opportunity for acceleration, For instance, model can be inferred in parallel, i.e., splitting the model into 2 parts and utilizing both CPU and GPU for inference. It may be promising, especially for those with multi-branch structure.
    Another opportunity is cloud-device co-design, which calibrates the existing compilation pipeline. Specifically, framework can fetch pre-compiled binaries to avoid cold-start issue, and apply JIT technique to adjust the compiled binaries. In such way, the binaries are optimized on-the-fly and constantly adapt to equipment.

    \textbf{For application developers.} Inspired from \textbf{F6}, \textbf{F7} and \textbf{F8}, Web application should be QoE-oriented, which means QoE has the highest priority. In other words, latency is not the only factor to consider. Take face detection in living scenario as an example, WebGL may outperforms wasm, but inference on GPU may make the screen stuck. In such case, leveraging wasm may bring better QoE, suggesting developers to select CPU as inference hardware. 
    % \yuanchun{In this implication, is there any guidelines for the dev to select backends? Also, is there any insight for whether to use in-browser inference instead of on-server inference?}

    % Since there is still huge gap between browser and the native, there are many possible optimization can be applied to in-browser inference scenario.
    % The first is kernel scheduling. Because there are 2 types of hardware available, it is possible to infer in parallel. For example, splitting the models into 2 parts and utilize both CPU and GPU for inference.
    % The second is kernel optimization. Although AOT compilation enables quick start, JIT can make compiled binaries more suitable for each hardware. This encourage developers to make a cloud-edge co-design approach to improve in-browser inference. For example, the framework can fetch pre-compiled binaries to avoid cold start problem, and apply JIT to optimize kernels.
\input{tex/tab-qoe-dl}

==> tex/introduction-deprecated.tex <==
\section{Introduction}
\label{sec:intro}

% \qipeng{
% ----------------------------------------story line--------------------------------------------
    
%     1. DNN has been a key enabler of modern applications, as a forward step, in-browser inference is promising, due to its sharability.
    
%     2. In-browser inference has not been well studied, except www' 2019. However, what is the detailed performance and how much is the optimization space has not been explored. Moreover, what will be brought to web users by deploying DL into browser, i.e. how the QoE will be?
    
%     3. our RQs: (i) explore inference in detail; (ii) explore the diversity/heterogeneity of user devices; (iii) explore the web QoE with DL deployment
    
%     4./5./6. For each RQ, summarize our experiment settings and findings
    
%     7. summarize implication of our work: for framework/model/web-app developer
    
% -------------------------------------------------------------------------------------------------------
% }
% \qipeng{
%     % on-device inference is good
%     % web application is good
%     % DL + browser is good!
    
%     In recent years, \emph{on-device inference} has been a new inference paradigm of deep learning (DL) and a key component of modern applications that are powered by deep neural network (DNN), such as input method assistant and voice recognition, etc~\cite{FLblog, apple-siri-blog, bonawitz2019towards}. Typical on-device inference runs in native applications, which introduce additional barriers to users due to installation and maintenance. 
%     \xucao{I think example scenarios don't seem to be strong driving cases for mobile DL, e.g. is there any demand for in-web Input Method?}
%     Meanwhile, web applications are emerging as their lightweight and convenience, because they do not require installation and maintenance for users. Benefiting from the cross-platform characteristic, web application does not require platform-specific adoption. Such advantages also lower the barrier for application developers.
%     \xucao{Does there exist any causality that on-device inference
%     calls for on-web inference, such as in certain domains? or they just get developed in parallel? And do we want to emphasize the connection? }
%     As a forward step, in-browser inference has been drawing attentions, which integrates DL into browser and performs inference in browser. In-browser inference will power many potential web applications, face detection for online meeting and typing assistant for online documentation.
% }

In recent years, a new inference paradigm, \emph{on-device inference} plays a key role in Deep Learning (DL) powered applications on end-user devices. There are numerous benefits associated with on-device inference, including 
%xucao ~ low interactive latency,
no network latency, accessibility
% \xucao{I think ``accessibility'' commonly comes with the meaning that helps people with physical disabilities -- is that what we are referring to?}
and data privacy.
% \xucao{ || Perhaps breaking paragraph here? ||}
% \xucao{START<<}
For native inference, typically inference frameworks, \eg TensorFlow~\cite{abadi2016tensorflow} and MNN~\cite{jiang2020mnn}, are required to be pre-installed. The indispensable Deep Neural Networks (DNN) have to be stored on device.
% \xucao{>>END I think these tasks are offloaded to app devs, not end-users. Suggest that like previous versions as well as you pointed out in the next paragraph, installation is the key barrier.} 
It definitely introduces additional barriers for end-users to access AI services on device.

% \xucao{how about ``In contrast (to native apps),''? and breaking into new paragraph as we introduce native apps above seems more structured}

Web browser is a promising platform for on-device inference. Without additional installations, DNNs and the framework can be encapsulated in a web application and delivered within web pages. Moreover benefiting from the cross-platform characteristic, web applications require no platform-specific adaption.
% \xucao{I feel it's less a \textit{benefit} -- could it prohibit certain adaptions? I think putting these two properties in parallel is enough }. 
These advantages are particularly important for both end-users and developers. As a result, DL inference in browsers would enhance and even enable many web applications.
% \xucao{I think it's kinda confusing how these becomes \textit{roots} and \textit{results}... How about: if we want to emphasize the functionality improvement because of web+DL, as a driving factor of our study, why not just remove ``As a result''?}
% On the other hand, integrates DL into browser and performs inference in browser. In-browser inference will power many potential web applications, face detection for online meeting and typing assistant for online documentation.
To facilitate DNN inference in web browsers, there are already several frameworks developed, \eg TensorFlow.js~\cite{tfjs} and ONNX Web Runtime~\cite{ortjs}. Such sophisticated frameworks are generally based on JavaScript.
% \xucao{DEL<<Such sophisticated frameworks are generally based on Javascript~\cite{}.>>DEL Consider removing, this statement doesn't seem helpful and such problems should be naturally overcame by any framework.}
To obtain better performance, modern  hardware acceleration backends are also adapted to access computation resources, \eg WebAssembly (wasm)~\cite{wasm} for CPU, WebGL~\cite{webgl} and WebGPU~\cite{webgpu} for GPU. 

% \xucao{Seems a little sudden -- why there is even a question? perhaps we need to tell some stories such as ``... but the performance of in-browser DL is magic and no one understands...''}

    A number of studies anatomize the DL performance on device~\cite{DeepBench, zhu2018benchmarking}. However, web browser is less considered. Because of the hardware abstraction in browser, hardware-specific features are often hidden to web applications. It makes the browser a unique platform for DL. Meanwhile, DNN is an unprecedented workload for web performance measurements. What the performance of \textit{in-browser inference} is and how much it brings to end-users has not been well studied.
% In this paper, we seek to answer the question that \emph{what is the detailed performance and the achieved user experience of the current in-browser DNN inference in real web applications}.  
% web applications lack the ability to leverage platform-specific features, it may lose opportunity to improve performance specially for certain device.
% For instance, WebAssembly (wasm) is a binary instruction format for a stack-based virtual machine, enabling running in browser more efficiently than pure JS, and WebGL can leverage the parallelism capacity of modern GPU to accelerate computing. These backends provide the ability to perform in-browser inference with high-performance.
    % few to measure DL@browser --> unknown facts
% There is still huge gap between the native and browser. In comparison, however, there are fewer studies considering deploying DL into browser. Most of existing studies consider and anatomize the performance of inference in native~\cite{DeepBench, zhu2018benchmarking}. These work provides the ability to profile the DL process in depth.
% However, when inferring models in browser, what is the detail performance and how large is the optimization room of in-browser inference has not been well studied. 
% As web application lacks the ability to leverage platform-specific features, it may lose opportunity to improve performance specially for certain device. On the other hand, user activities may cause resource competition, leading to pool inference performance in resource-constrained browsers. What is the diversity of user devices and activities are not well studied yet.
% Web browsing is a activity where quality of experience (QoE) has the hightest priority. Deploying DL into browser will bring more opportunities to enable diverse applications, thus, improving the QoE.
% \xucao{the QoE rooted in more diverse apps seems to be about functionality, is it the same as the QoE that is measuring, say, the "smoothness" of the browsing?}
% However, different from traditional browsing which consider more about loading, what is QoE during DL inference has not been well studied.
% \qipeng{
To fill this gap, we make the first measurement study to demystify DNN inference in browser. We have the following research questions:
    % \begin{itemize}[leftmargin=*,nosep]
    %     \item \textbf{RQ1}: what is the detailed performance and how large is the gap between the native and browser, what are the root causes?
        
    %     \item \textbf{RQ2}: what is the inference performance distribution among user devices?
        
    %     \item \textbf{RQ3}: what is the QoE during DL inference?
    % \end{itemize}
    % We conduct extensive experiments for each RQ, and summarize our results and findings.
% }


    % \textbf{RQ1}
    \textbf{RQ1}(\S\ref{sec:performance}): \textit{what is the detailed performance and how large is the gap between the native and browser inference, what are the root causes?}
    
    We select 2 frameworks, i.e., TensorFlow.js (tf.js) and ONNX Web Runtime (ort.js), as well as their native counterparts.
    % \xucao{\underline{version} counterparts -- seems no direct native distributions are there for tfjs etc.}, 
    % i.e. TensorFlow (tf) and ONNX Runtime (ort). We select 15 typical DNN models. \xucao{DEL<<We measure the end-to-end performance and make a breakdown analysis of the inference process. We also profile the inference process in detail.>>DEL
    We profile the end-to-end inference process in detail and make a breakdown analysis, we have the following results:
    
    As for latency, there is still large gap between the native and browser, and the latency pattern are different between 2 scenarios. We breakdown the inference into different stages and measure the latency of each stage. 
    % \xucao{DEL<<We find in different stage, each framework and backend performs differently.>>DEL We find in all (or just some?) stages, different frameworks and backends perform differently.}
    We summarize the root cause of the performance gap, such as weight transformation overhead and hardware preparation overhead, etc. 
    We then zoom into the acceleration methods on CPU, 
    %xucao:
    %and analyze the contributions of different acceleration methods, including multi-thread and Single Instruction Multiple Data (SIMD). We find that both methods contribute to acceleration significantly.
    namely multi-thread and Single Instruction Multiple Data (SIMD), 
    and find both methods contribute to acceleration significantly.
    % \xucao{in which way generally? how about ``significantly''?}.
    To further understand the latency, we also profile and analyze the inference in kernel-level. We find that there exist kernels dominating the overall latency. An interesting result is that multi-thread may degrade the performance of memory-intensive kernel in wasm backend. We also anatomize the underlying mechanism and summarize the cause.

    As for memory footprint, it can be a bottleneck of inference in web browsing scenarios.
    % although its priority is lower than latency\xucao{any reason for this inferiority? would it be ``... in web browsing scenarios''?}, it can still be a bottleneck of in-browser inference.}
    We profile the memory footprint during inference in kernel-level, and find that inference process may crush due to high memory usage, especially on GPU. We dive into the memory access patterns of different models, and find this may be a common phenomenon for super-resolution models like GAN~\cite{wang2018esrgan}.



    \textbf{RQ2} (\S\ref{sec:large-scale}): \textit{what is the inference performance distribution among diverse user devices?} 
    
    We develop a benchmark application to collect device hardware specifications, monitor system state and resource utilization, drive in-browser inference and collect the profiled data. We distribute the application and collect data from 50 volunteers. 
    
    We analyze inter- and intra-device diversity. For inter-device diversity, we find that the end-to-end latency varies. Even for the same model, the latency would vary up to 1.73$\times$. We analyze the resource utilization as well as hardware capacity, and conclude that hardware capacity dominates the latency. For intra-device diversity, we analyze the data from each device, and also find that the latency varies, but not as much as that of inter-device. The reason is resource competition from other processes. These results indicate that the heterogeneity of runtime environment significantly impacts the inference performance, encouraging developers to design optimizations that can fit more scenarios.



    \textbf{RQ3} (\S\ref{sec:qoe}): \textit{what is the user experience during inference in browsers?} 
    
    Traditional QoE metrics~\cite{speedindex, PLT} for web browsing are not suitable for in-browser inference scenarios. We redefine QoE during inference and design experiments to quantify it judiciously. Specifically, for 3 aspects: (1) responsiveness of web page, i.e., how timely the response is when the user interacts with the web page; (2) fluency of web page, i.e., how fluent is the web page rendered or video played during inference; (3) DL performance, i.e., what the DL performance on a certain web application compared with the native. We find that deploying DL into browser will inevitably degrade the responsiveness and fluency of web page. When inferring model on integrated GPU, fluency drops much more than other scenarios. As for DL performance, we find that although inference on GPU is faster than inference on CPU, CPU may outperform GPU with respect to DL performance on a certain application. The reason is inference on GPU may make the web page stuck, leading to poor model performance.
    %\xucao{SKIP SKIP SKIP I think the case GPU inference hurts model performance -- of course we keep saying execution performance, but is this about numerical solution accuracy? -- is a particularly surprising observation, suggest adding some more details, like ``... stuck the web  page, which is the source of model inputs, leading ... certain apps like face detection.''}



    % \textbf{Implications.}
    Our study derives insightful implications for various stakeholders. For framework developers, there are several optimization opportunities. For example, frameworks can enable kernel specialization and optimization for different hardware architectures, since kernel performance varies significantly among devices, and different kernels may prefer different acceleration methods, like multi-thread and SIMD. Memory management is also critical when inferring models with specific model structures, especially for limited GPU memory. Inferring model in parallel is a promising way which can maximize the role of multi-thread, especially for model with multi-branch structure. For application developers, QoE should be the factor with the highest priority that should be considered. Application should not exhaust all available resources to guarantee solely inference performance, but reserve sufficient resources to ensure the performance of other tasks.
    % \xucao{would you think this is quite high-level? For example, do we have certain aspects that are building blocks of QoE for devs to care about, such as heterogeneous hardware utilization and, perhaps, user-flow-level redesign?}
    Take video application developers as an example, inference on CPU may be more suitable for devices with limited GPU capacity, because fluency depends on GPU.



    We summarize our contributions as following:
    \begin{itemize}[leftmargin=*,nosep]
        \item We present the first measurement study to demystify DNN inference in detail, and conduct measurement on amount of user devices to explore the diversity of user devices.
        \item We define the QoE during inference and conduct experiment to quantify it. Experiment results show the gap between better QoE and better inference performance.
        \item We develop an benchmark application that can profile in-browser inference, monitor system state automatically. The code would be open-sourced. 
        % once the paper is accepted.
    \end{itemize}

==> tex/measurements.tex <==
\section{Inference Performance among diverse User Devices}
\label{sec:large-scale}

\input{tex/fig-inter-latency-distribution}

% \subsubsection{Ethic Consideration}
% Our work is approved by the Research Ethical Committee of authors' institutes. The volunteers are informed with explicit user-term statements. We collect the data via the automatic application, which does not require any additional support from the device. We follow a strict policy in data collection and storage. During the collection process, the application does not collect any personal private data, i.e., only hardware information, profiled inference data, and monitored system state are collected. The server, where service is deployed and data is stored, is located in LAN with strict authentication and access mechanism. We use the hash of the device IP in LAN to identify each device (192.169.XX.XX), to ensure anonymization. 



\subsection{Inter-device diversity.}\label{subsubsec:inter-device}

Figure~\ref{fig:inter-latency-distribution} illustrates the inference latency distribution of the models. We can see that the inference latency of each model varies differently among devices.
Take ResNet50 in the wasm backend as an example, the three quartiles of its inference latency are 257.6ms, 358.4ms, and 680.9ms, respectively. The latency variance reaches up to 28.40$\times$, indicating that the inter-device latency spans a wide spectrum. Such diversity derives from different hardware capacities. The frequency and core number of different CPUs vary diversely. For example, we consult the data from the CPU benchmark website and compared it with the hardware information collected in our dataset. We observe that the lowest-end CPU in our dataset, Core i5 Skylake, had a score of 4.1$\times$ lower than the highest-end CPU, Core i7 Rocket Lake (6030 vs. 24673)~\cite{cpu-benchmark, cpubenchmark-i5-6gen, cpubenchmark-i7-11gen}.


Additionally, it's important to note that user activities can have an impact on inference performance. We find that not all inference processes can effectively utilize CPU resources, primarily due to the presence of background applications during inference. For instance, when inferring the ResNet50 model on an idle device (as described in \S\ref{sec:performance}), the normalized CPU utilization of the inference process can reach 55\%. However, when considering the average CPU utilization across user devices, the normalized average utilization is only around 30\%. This lower CPU utilization can primarily be attributed to resource competition. When there are other active applications running concurrently with the inference process, the CPU resources available for the inference task become limited, preventing it from fully utilizing all available CPU resources.


\subsection{Intra-device diversity.}\label{subsubsec:intra-device}

To gain further insights into the impact of resource competition, we conduct intra-device experiments. Within a single device, we observe that inference latency can vary due to different runtime environments, such as whether the device is idle or not. We select the device with the most data points for our analysis. As obtaining GPU utilization data of a certain process proved challenging, we focus on examining the relationship between CPU utilization and inference latency. 
Figure~\ref{fig:intra-latency+utilization-distribution} illustrates the inference latency distribution of the models, as well as the corresponding CPU utilization of inferring process. 
We can see that the latency and utilization also vary (e.g., up to 1.73$\times$ for SSD-MobileNetV2), but not as significantly as the results shown in Figure~\ref{fig:inter-latency-distribution}. 
The observed variation can primarily be attributed to diverse CPU utilization, which, in turn, stems from resource competition among different applications running on the device. 


An intriguing observation emerges when considering the latency of certain models, such as MobileNetV2, in relation to varying levels of CPU utilization. Despite significant fluctuations in CPU utilization, the latency of these models remains relatively stable. This phenomenon can be attributed to the fact that MobileNetV2 and similar models involve a smaller number of computational kernels compared to other models. Consequently, the inference latency of these models is inherently low. Such a finding indicates that even in scenarios where CPU utilization experiences a slight fluctuation, its impact on latency is relatively insignificant.
Furthermore, our observation reveals an interesting insight regarding the potential of multi-threading for accelerating MobileNetV2. We find that when enabling multi-threading on an idle device with four cores, the normalized CPU utilization for MobileNetV2 hovers just above 25\%. This modest utilization level indicates that the acceleration gains achieved through multi-threading are relatively limited for this particular model. Consequently, any decrease in CPU utilization has only a marginal effect on the latency of MobileNetV2, further highlighting the model's resilience to changes in CPU workload. This finding is consistent with the results presented in \S\ref{sec:performance}. In \S\ref{subsubsec:e2e-latency-analysis}, we observe that SIMD technology brings more acceleration in MobileNetV2 inference than multi-threading.

% \input{tex/fig-intra-latency+utilization-distribution}

\finding{
    \textbf{Finding 4 (\S\ref{subsubsec:inter-device})}: the inference latency can exhibit significant variations across different devices. This discrepancy in latency can be attributed to the divergence in device capacities. In our experiments, we observe a maximum gap of 28.4$\times$ in the wasm backend and 19.4$\times$ in the WebGL backend. Such considerable variance among devices emphasizes the need to account for device capacity divergence and optimize models and frameworks accordingly. By acknowledging and addressing these disparities, developers can ensure that the applications perform optimally across a wide range of devices, delivering consistent and satisfactory service.
    \\
    \textbf{Finding 5 (\S\ref{subsubsec:intra-device})}: even within the same device (intra-device), the inference latency can still exhibit variations. In our experiments, we observe differences of up to 1.73$\times$ in latency for the same model. These results highlight developers cannot assume that inference tasks will fully utilize all available resources. Factors such as runtime environment, resource competition, and other active applications on the device can impact the extent to which resources are effectively utilized. It is crucial for developers to consider these variations and design models and applications accordingly, taking into account potential resource limitations and optimizing for optimal performance under diverse conditions.
}



==> tex/tab-dnn-distribution.tex <==
\begin{table*}[]

    \caption{Inference accuracy on certain applications. The format of each entry, ``/'', ``-D/-I'', and ``M*'' keeps the same as Table~\ref{tab:qoe-merge}.}
    \label{tab:qoe-dl}
    \vspace{-4mm}
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lrrrrrr}
    \toprule[1.5pt]
                   & \multicolumn{1}{c}{M1}               & \multicolumn{1}{c}{M2}               & \multicolumn{1}{c}{M3}              & \multicolumn{1}{c}{M4}                & \multicolumn{1}{c}{M5}                & \multicolumn{1}{c}{M6} \\ \hline
    TF.js-Wasm      & 13.7\% (0.53$\times10^{-2}$)         & 13.5\% (0.52$\times10^{-2}$)         & 8.8\% (0.33$\times10^{-2}$)         & 0.78 (2.91$\times10^{-2}$)            & /                                     & /                              \\
    ORT.js-Wasm    & 13.7\% (0.50$\times10^{-2}$)         & 13.6\% (0.52$\times10^{-2}$)         & 8.0\% (0.30$\times10^{-2}$)         & 0.78 (3.10$\times10^{-2}$)            & 0.77 (2.84$\times10^{-2}$)            & 0.79 (3.00$\times10^{-2}$)     \\
    TF.js-WebGL-I   & 8.7\%  (0.33$\times10^{-2}$)         & 8.8\%  (0.32$\times10^{-2}$)         & 3.9\% (0.14$\times10^{-2}$)         & 0.76 (2.86$\times10^{-2}$)            & 0.76 (2.93$\times10^{-2}$)            & 0.78 (2.83$\times10^{-2}$)     \\
    TF.js-WebGL-D   & 14.9\% (0.54$\times10^{-2}$)         & 14.2\% (0.52$\times10^{-2}$)         & 11.1\% (0.44$\times10^{-2}$)        & 0.95 (3.26$\times10^{-2}$)            & 0.94 (3.41$\times10^{-2}$)            & 0.96 (3.59$\times10^{-2}$)     \\
    ORT.js-WebGL-I & 10.5\% (0.39$\times10^{-2}$)         & 11.1\% (0.45$\times10^{-2}$)         & 7.9\% (0.30$\times10^{-2}$)         & /                                     & /                                     & /                              \\
    ORT.js-WebGL-D & 15.1\% (0.57$\times10^{-2}$)         & 15.1\% (0.56$\times10^{-2}$)         & 13.5\% (0.54$\times10^{-2}$)        & /                                     & /                                     & /                              \\ \bottomrule[1.5pt]
    \end{tabular}%
    }

\end{table*}

==> tex/tab-e2e-ort-webgl.tex <==
\begin{table*}[tp]
    \centering
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{@{}l|rrrrrrrrrrrr@{}}
    \toprule[1.5pt]
                                & \multicolumn{3}{c|}{Wasm}                                                               & \multicolumn{3}{c|}{Wasm-thread}                                                        & \multicolumn{3}{c|}{Wasm-SIMD}                                       & \multicolumn{3}{c}{Wasm-thread-SIMD}                                                   \\ \cmidrule(l){2-13} 
                                & \multicolumn{1}{c}{setup} & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c|}{inference} & \multicolumn{1}{c}{setup} & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c|}{inference} & setup  & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c|}{inference} & \multicolumn{1}{c}{setup} & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c}{inference} \\ \midrule
    (M1) MobilenetV2          & 581.4                     & 120.1                      & 148.6                          & 1306.6                    & 216.9                      & 122.4                          & 1252.1 & 162.8                      & 106.5                          & 331.0                     & 139.6                      & 105.5                         \\
    (M2) Resnet50             & 539.3                     & 1299.5                     & 1275.3                         & 699.1                     & 394.1                      & 395.7                          & 2412.3 & 411.9                      & 358.1                          & 1219.3                    & 306.9                      & 172.3                         \\
    (M3) VGG16                & 7545.3                    & 9024.7                     & 8275.6                         & 4437.5                    & 8147.2                     & 8140.1                         & 2695.2 & 3164.6                     & 2947.2                         & 2423.2                    & 1353.6                     & 1334.1                        \\
    (M4) SSD-MobilenetV2      & 1120.5                    & 279.6                      & 287.4                          & 1338.1                    & 197.3                      & 123.9                          & 1171.8 & 174.5                      & 126.1                          & 1467.8                    & 81.5                       & 84.4                          \\
    (M5) EfficientDet          & 1581.2                    & 2665.4                     & 2648.6                         & 1786.4                    & 1251.6                     & 1282.5                         & 1606.1 & 1245.8                     & 1228.8                         & 1889.6                    & 852.0                      & 926.4                         \\
    (M6) Yolo5-Middle          & 427.6                     & 1105.2                     & 1092.7                         & 450.0                     & 365.9                      & 362.9                          & 408.1  & 406.2                      & 386.4                          & 457.6                     & 145.8                      & 145.2                         \\
    (M7) USE                  & 744.6                     & 915.2                      & 910.2                          & 702.4                     & 279.8                      & 285.6                          & 681.8  & 246.2                      & 247.2                          & 574.8                     & 92.8                       & 81.6                          \\
    (M8) MobileBert-Base      & 873.5                     & 849.1                      & 855.8                          & 935.8                     & 291.1                      & 310.1                          & 865.0  & 236.3                      & 239.2                          & 945.0                     & 120.2                      & 113.6                         \\
    (M9) Bert-Small           & 155.2                     & 21.2                       & 21.8                           & 161.3                     & 9.2                        & 7.8                            & 158.1  & 7.1                        & 6.7                            & 166.8                     & 4.6                        & 4.7                           \\
    \bottomrule[1.5pt]
    \end{tabular}%
    }
    \caption{Latency (ms) of models in ort.js wasm backend. ``-SIMD/thread" indicates enabled technique.}
    \label{tab:e2e-ort-wasm}
    \vspace{-4mm}
\end{table*}

==> tex/tab-e2e-tfjs-webgl.tex <==
\begin{table}[tp]
\centering
\scriptsize
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{l|rrrrrr}
\toprule[1.5pt]
    & \multicolumn{3}{c|}{tf.js-WebGL-I}                                                       & \multicolumn{3}{c}{tf.js-WebGL-D}                                                       \\ \cline{2-7} 
    & \multicolumn{1}{c}{setup} & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c|}{inference} & \multicolumn{1}{c}{setup} & \multicolumn{1}{c}{warmup} & \multicolumn{1}{c}{inference} \\ \hline
M1  & 209.5                     & 2900.7                     & 28.7                           & 530.9                     & 5751.0                     & 20.1                          \\
M2  & 1635.7                    & 2814.2                     & 248.3                          & 2482.7                    & 5443.6                     & 79.8                          \\
M3  & 503.1                     & 7047.6                     & 1039.0                         & 1125.2                    & 15097.9                    & 616.6                         \\
M4  & 480.0                     & 5240.8                     & 212.1                          & 1243.5                    & 10483.6                    & 77.0                          \\
M5  & 443.5                     & 5230.3                     & 396.5                          & 999.2                     & 9795.3                     & 115.9                         \\
M6  & 1902.7                    & 3126.1                     & 682.0                          & 3412.0                    & 3128.2                     & 133.4                         \\
M7  & 2837.3                    & 3169.5                     & 943.1                          & 3538.0                    & 2196.4                     & 400.5                         \\
M8  & 664.0                     & 2089.0                     & 41.1                           & 839.3                     & 2273.4                     & 58.3                          \\
M9  & 9109.0                    & 3414.5                     & 1748.7                         & 10090.0                   & 4719.0                     & 913.9                         \\
M10 & 426.5                     & 2057.6                     & 38.0                           & 731.5                     & 3458.4                     & 23.5                          \\
M11 & 1666.8                    & 3457.0                     & 535.5                          & 2925.7                    & 6009.6                     & 121.2                         \\
M12 & 15568.8                   & 4515.5                     & 53.3                           & 2938.5                    & 9847.1                     & 44.0                          \\
M13 & 1739.7                    & 5796.1                     & 99.4                           & 2054.3                    & 10873.6                    & 82.9                          \\
M14 & 550.5                     & 4416.0                     & 393.7                          & 1193.3                    & 7492.2                     & 115.9                         \\
M15 & 734.8                     & 26235.6                    & 11736.1                        & 2542.3                    & 38127.3                    & 2955.6                        \\
M16 & 4193.5                    & 8395.2                     & 2098.9                         & 2032.8                    & 10705.3                    & 1264.7                        \\ \bottomrule [1.5pt]
\end{tabular}%
}
\caption{Latency (ms) of models in tf.js WebGL backend. ``-I/-D'' indicates integrated/discrete GPU. ``M*'' is the model ID; it is consistent with Table~\ref{tab:e2e-native-all}.}
\label{tab:e2e-tfjs-webgl}
\vspace{-4mm}
\end{table}

==> tex/tab-qoe-merge.tex <==
\begin{table*}[]
    \caption{Partial results of QoE. Each entry is in the format of ``mean (standard deviation)''. ``/'' indicates the model is not supported. ``-D/-I'' denotes the discrete/integrated GPU. ``M*'' denotes model ID and is consistent with \S\ref{subsec:experimental_setup}.} 
    \label{tab:qoe-merge}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{l|rrr|rrr|rr}
        \toprule[1.5pt]
                       & \multicolumn{3}{c|}{Rresponsiveness}                                                          & \multicolumn{3}{c|}{Smoothness}                                                                  & \multicolumn{2}{c}{Inference accuracy}                                                  \\ \cline{2-9} 
                       & \multicolumn{1}{c}{M1}         & \multicolumn{1}{c}{M4}        & \multicolumn{1}{c|}{M7}      & \multicolumn{1}{c}{M1}         & \multicolumn{1}{c}{M4}        & \multicolumn{1}{c|}{M7}         & \multicolumn{1}{c}{M1}                        & \multicolumn{1}{c}{M4}                  \\ \hline
        Baseline       & 142.0 \ \ (2.3)                & 142.0 \ \ (2.3)               & 142.0 \ \ (2.3)              & 30.0 (0.00)                    & 30.0 (0.00)                   & 60.0 (0.00)                     & 17.2\% (0.00)\quad \quad \ \ \                & 1.00 (0.00)\quad \quad \ \ \            \\
        TF.js-wasm     & 92.7 \ \ (7.5)                 & 112.0 \ \ (7.0)               & /                            & 23.8 (1.83)                    & 23.9 (1.65)                   & /                               & 13.7\% (0.53$\times10^{-2}$)                  & 0.78 (2.91$\times10^{-2}$)              \\
        ORT.js-wasm    & 92.0 \ \ (5.0)                 & 108.0 (11.0)                  & 92.1 (6.6)                   & 24.1 (1.79)                    & 23.8 (1.79)                   & 54.6 (4.07)                     & 13.7\% (0.50$\times10^{-2}$)                  & 0.78 (3.10$\times10^{-2}$)              \\
        TF.js-WebGL-I  & 87.6 (12.0)                    & 113.0 (13.0)                  & 89.3 (9.5)                   & 11.2 (0.77)                    & 12.7 (0.82)                   & 26.8 (2.10)                     & 8.7\%  (0.33$\times10^{-2}$)                  & 0.76 (2.86$\times10^{-2}$)              \\
        TF.js-WebGL-D  & 118.1 \ \ (2.9)                & 127.4 \ \ (7.4)               & 113.5 (3.1)                  & 27.2 (1.29)                    & 28.3 (1.71)                   & 52.4 (2.44)                     & 14.9\% (0.54$\times10^{-2}$)                  & 0.95 (3.26$\times10^{-2}$)              \\
        ORT.js-WebGL-I & 89.7 \ \ (7.7)                 & /                             & /                            & 17.0 (1.11)                    & /                             & /                               & 10.5\% (0.39$\times10^{-2}$)                  & /                                       \\
        ORT.js-WebGL-D & 123.1 \ \ (5.1)                & /                             & /                            & 26.4 (1.39)                    & /                             & /                               & 15.1\% (0.57$\times10^{-2}$)                  & /                                       \\ \bottomrule[1.5pt]
        \end{tabular}%
    }
    \vspace{-4mm}
\end{table*}

==> tex/tab-responsiveness-mean-distribution.tex <==
\begin{table*}[]
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lrrrrrrrrr}
        \toprule[1.5pt]
                       & \multicolumn{1}{c}{M1}       & \multicolumn{1}{c}{M2}   & \multicolumn{1}{c}{M3} & \multicolumn{1}{c}{M4}   & \multicolumn{1}{c}{M5}   & \multicolumn{1}{c}{M6}   & \multicolumn{1}{c}{M7}     & \multicolumn{1}{c}{M8}   & \multicolumn{1}{c}{M9} \\ \hline
        tfjs-wasm      & 92.7 \ \ (7.5)               & 89.5 (11.0)              & 91.2 (7.0)             & 112.0 \ \ (7.0)          & /                        & /                        & /                          & /                        & /                      \\
        ort.js-wasm    & 92.0 \ \ (5.0)               & 94.5 \ \ (9.2)           & 88.4 (9.8)             & 108.0 (11.0)             & 92.6 (12.0)              & 91.0 \ \ (7.0)           & 92.1 (6.6)                 & 115.0 (12.2)             & 83.7 \ \ (7.0)         \\
        tfjs-WebGL-I   & 87.6 (12.0)                  & 84.2 \ \ (7.5)           & 94.2 (8.3)             & 113.0 (13.0)             & 100.4 \ (9.3)            & 97.4 (11.2)              & 89.3 (9.5)                 & 106.0 \ \ (7.7)          & 83.1 (12.5)            \\
        tfjs-WebGL-D   & 118.1 \ \ (2.9)              & 119.2\ \ \ (3.8)         & 114.5 (3.6)            & 127.4 \ \ (7.4)          & 121.3 \ (6.3)            & 112.0 \ \ (2.4)          & 113.5 (3.1)                & 120.8 \ \ (3.6)          & 95.5 \ \ (8.6)         \\
        ort.js-WebGL-I & 89.7 \ \ (7.7)               & 88.2 \ \ (8.4)           & 96.2 (4.4)             & /                        & /                        & /                        & /                          & /                        & /                      \\
        ort.js-WebGL-D & 123.1 \ \ (5.1)              & 119.7\ \ \ (6.2)         & 125 (4.0)              & /                        & /                        & /                        & /                          & /                        & /                      \\ \bottomrule[1.5pt]
                           
    \end{tabular}%
    }

    \caption{The average and standard deviation of the responsiveness mean score. We get the mean score on each device, and then calculate the average and the standard deviation of all mean scores.
    Each entry of the table is in the format of ``average (standard deviation)''. ``/'' indicates the model is not supported. ``-D/-I'' indicates the discrete or integrated GPU. ``M*'' is the model ID and is consistent with Table~\ref{tab:e2e-native-all} in the draft.}
    \label{tab:responsiveness-mean-distribution}
\end{table*}
    
    % The score is obtained from Speedometer

==> tex/tab-responsiveness-std-distribution.tex <==
\begin{table*}[]
    \resizebox{0.95\linewidth}{!}{%
    \begin{tabular}{lrrrrrrrrr}
        \toprule[1.5pt]
                       & \multicolumn{1}{c}{M1}       & \multicolumn{1}{c}{M2}   & \multicolumn{1}{c}{M3} & \multicolumn{1}{c}{M4}   & \multicolumn{1}{c}{M5}   & \multicolumn{1}{c}{M6}   & \multicolumn{1}{c}{M7}     & \multicolumn{1}{c}{M8}   & \multicolumn{1}{c}{M9} \\ \hline
        tfjs-wasm      & 92.7 \ \ (7.5)               & 89.5 (11.0)              & 91.2 (7.0)             & 112.0 \ \ (7.0)          & /                        & /                        & /                          & /                        & /                      \\
        ort.js-wasm    & 92.0 \ \ (5.0)               & 94.5 \ \ (9.2)           & 88.4 (9.8)             & 108.0 (11.0)             & 92.6 (12.0)              & 91.0 \ \ (7.0)           & 92.1 (6.6)                 & 115.0 (12.2)             & 83.7 \ \ (7.0)         \\
        tfjs-WebGL-I   & 87.6 (12.0)                  & 84.2 \ \ (7.5)           & 94.2 (8.3)             & 113.0 (13.0)             & 100.4 \ (9.3)            & 97.4 (11.2)              & 89.3 (9.5)                 & 106.0 \ \ (7.7)          & 83.1 (12.5)            \\
        tfjs-WebGL-D   & 118.1 \ \ (2.9)              & 119.2\ \ \ (3.8)         & 114.5 (3.6)            & 127.4 \ \ (7.4)          & 121.3 \ (6.3)            & 112.0 \ \ (2.4)          & 113.5 (3.1)                & 120.8 \ \ (3.6)          & 95.5 \ \ (8.6)         \\
        ort.js-WebGL-I & 89.7 \ \ (7.7)               & 88.2 \ \ (8.4)           & 96.2 (4.4)             & /                        & /                        & /                        & /                          & /                        & /                      \\
        ort.js-WebGL-D & 123.1 \ \ (5.1)              & 119.7\ \ \ (6.2)         & 125 (4.0)              & /                        & /                        & /                        & /                          & /                        & /                      \\ \bottomrule[1.5pt]
                           
    \end{tabular}%
    }

    \caption{The average and standard deviation of the responsiveness score standard deviation. We get the score standard deviation on each device, and then calculate the average and the standard deviation of all standard deviations.
    Each entry of the table is in the format of ``average (standard deviation)''. ``/'', ``-D/-I'', and ``M*'' indicate the same as Table~\ref{tab:responsiveness-mean-distribution}.}
    \label{tab:responsiveness-std-distribution}
\end{table*}
    
    % The score is obtained from Speedometer

==> tex/tab-smoothness-distribution.tex <==
\begin{table*}[]

    \caption{Smoothness of Web page. The format of each entry, ``/'', ``-D/-I'', and ``M*'' keeps the same as Table~\ref{tab:qoe-merge}.}
    \label{tab:qoe-fps}
    \vspace{-4mm}
    \resizebox{0.95\linewidth}{!}{%
        \begin{tabular}{lrrrrrrrrr}
        \toprule[1.5pt]
                       & \multicolumn{1}{c}{M1} & \multicolumn{1}{c}{M2}         & \multicolumn{1}{c}{M3}         & \multicolumn{1}{c}{M4} & \multicolumn{1}{c}{M5}      & \multicolumn{1}{c}{M6}    & \multicolumn{1}{c}{M7} & \multicolumn{1}{c}{M8} & \multicolumn{1}{c}{M9}    \\ \hline
        TF.js-wasm      & 23.8 (1.83)            & 22.9 (1.79)                    & 22.4 (1.61)                    & 23.9 (1.65)            & /                           & /                         & /                      & /                      & /                         \\
        ORT.js-wasm    & 24.1 (1.79)            & 23.1 (1.49)                    & 24.5 (1.71)                    & 23.8 (1.79)            & 21.7 (1.66)                 & 22.4 (1.66)               & 54.6 (4.07)            & 53.7 (3.71)            & 52.7 (3.51)               \\
        TF.js-WebGL-I   & 11.2 (0.77)            & 11.7 (0.85)                    & 12.9 (1.01)                    & 12.7 (0.82)            & 11.1 (0.84)                 & 11.5 (0.79)               & 26.8 (2.10)            & 27.2 (1.82)            & 23.5 (1.73)               \\
        TF.js-WebGL-D   & 27.2 (1.29)            & 26.4 (1.18)                    & 28.1 (1.51)                    & 28.3 (1.71)            & 27.9 (1.26)                 & 28.1 (1.49)               & 52.4 (2.44)            & 51.5 (3.19)            & 52.0 (2.85)               \\
        ORT.js-WebGL-I & 17.0 (1.11)            & 16.8 (1.11)                    & 17.1 (1.31)                    & /                      & /                           & /                         & /                      & /                      & /                         \\
        ORT.js-WebDL-D & 26.4 (1.39)            & 23.0 (1.08)                    & 24.5 (1.14)                    & /                      & /                           & /                         & /                      & /                      & /                         \\ \bottomrule[1.5pt]
        \end{tabular}%
    }

\end{table*}

==> tex/tab-tfjs-kernel-proportion-merged.tex <==
\begin{table*}[t]
    \begin{tabular}{lrrrr|lrr}
    \hline
    Kernel        & wasm   & wasm-S & wasm-T & wasm-S-T & Kernel      & WebGL-I & WebGL-D \\ \hline
    Einsum        & 48.2\% & 46.5\% & 48.0\% & 41.4\%   & FusedConv2D & 43.6\%  & 23.7\%  \\
    FusedConv2D   & 47.6\% & 44.3\% & 47.4\% & 34.6\%   & Einsum      & 37.1\%  & 48.4\%  \\
    Gather        & 1.3\%  & 3.9\%  & 1.5\%  & 12.5\%   & Add         & 4.3\%   & 7.9\%   \\
    Slice         & 0.3\%  & 1.1\%  & 0.3\%  & 2.8\%    & Multiply    & 3.5\%   & 3.4\%   \\
    FusedDwConv2D & 1.3\%  & 1.2\%  & 1.3\%  & 1.9\%    & FusedMatMul & 2.3\%   & 2.9\%   \\ \hline
    \end{tabular}
    \caption{Tf.js top5 kernel latency average proportion in different backends. ``-S/T" indicates enabling SIMD/multi-thread. ``Dw" means ``Depthwise".
    Cell color red means the latency is a little longer than that of wasm (increment <5\%); yellow means the latency is close to that of wasm (difference <1\%); green means the latency is much less than that of wasm (decrement >10\%).}
\label{tab:merged}
\end{table*}

==> tex/tab-tfjs-top5kernel-latency-proportion.tex <==
\begin{table}[t]
  \caption{Top-5 kernels prediction latency proportion in TF.js. ``Dw'' denotes Depthwise. We enable SIMD and set 4 threads in Wasm. Each entry is the kernel prediction latency percentage out of the total latency of all models}
  \label{tab:tfjs-top5kernel-latency-proportion}
  \centering
  \begin{tabular}{lr|lr|lr}
    \toprule[1.5pt]
    Kernel        & Proportion & Kernel      & Proportion & Kernel      & Proportion \\ \hline
    Einsum        & 41.4\%     & FusedConv2D & 43.6\%     & Einsum      & 48.4\%     \\
    FusedConv2D   & 34.6\%     & Einsum      & 37.1\%     & FusedConv2D & 23.7\%     \\
    GatherV2      & 12.5\%     & Add         & 4.3\%      & Add         & 7.9\%      \\
    Slice         & 2.8\%      & Multiply    & 3.5\%      & Multiply    & 3.4\%      \\
    FusedDwConv2D & 1.9\%      & FusedMatMul & 2.3\%      & FusedMatMul & 2.9\%      \\ \bottomrule[1.5pt]
    \end{tabular}
  \vspace{-4mm}
\end{table}

==> tex/tab-tfjs-wasm-breakdown-kernel-latency-proportion.tex <==
\begin{table}[t]
    \caption{Breakdown analysis of the impact of different acceleration approaches in Wasm backend, the framework is TF.js. ``-S/T'' indicates SIMD/multithreading. ``Dw'' indicates ``Depthwise''. Each entry is the kernel prediction latency proportion.
    Cell color gray means the latency is a little longer than that of Wasm (1\%< increment <5\%); yellow means the latency is close to that of Wasm (difference <1\%); blue means the latency is much less than that of Wasm (decrement >10\%).}
    \label{tab:tfjs-wasm-breakdown-kernel-latency-proportion}
    \begin{tabular}{lrrrr}
        \toprule[1.5pt]
                                           & Wasm   & Wasm-S                         & Wasm-T                         & Wasm-S-T                       \\ \hline
        \multicolumn{1}{l|}{FusedConv2D}   & 47.6\% & \cellcolor[HTML]{34CDF9}44.3\% & \cellcolor[HTML]{34CDF9}47.4\% & \cellcolor[HTML]{34CDF9}34.6\% \\
        \multicolumn{1}{l|}{EinSum}        & 48.2\% & \cellcolor[HTML]{34CDF9}46.5\% & \cellcolor[HTML]{34CDF9}48.0\% & \cellcolor[HTML]{34CDF9}41.4\% \\
        \multicolumn{1}{l|}{Gather}        & 1.3\%  & \cellcolor[HTML]{F8FF00}3.9\%  & \cellcolor[HTML]{C0C0C0}1.5\%  & \cellcolor[HTML]{C0C0C0}12.5\% \\
        \multicolumn{1}{l|}{FusedMatMul}   & 0.8\%  & \cellcolor[HTML]{34CDF9}1.8\%  & \cellcolor[HTML]{34CDF9}0.8\%  & \cellcolor[HTML]{34CDF9}1.6\%  \\
        \multicolumn{1}{l|}{Slice}         & 0.3\%  & \cellcolor[HTML]{F8FF00}1.1\%  & \cellcolor[HTML]{C0C0C0}0.3\%  & \cellcolor[HTML]{C0C0C0}2.8\%  \\
        \multicolumn{1}{l|}{FusedDwConv2D} & 1.3\%  & \cellcolor[HTML]{34CDF9}1.2\%  & \cellcolor[HTML]{34CDF9}1.3\%  & \cellcolor[HTML]{34CDF9}1.9\%  \\ 
        \bottomrule[1.5pt]
        \end{tabular}
    \vspace{-4mm}
    \end{table}

==> tex/tab-tmp.tex <==
\begin{table*}[h]

    \caption{The fps standard deviation of the Web page. ``/'', ``-D/-I'', and ``M*'' indicate the same as the draft.}
    \vspace{-3mm}
    \label{tab:tmp}
    \centering
    \normalsize
        \begin{tabular}{lrrrrrrrrr}
        \toprule[1.5pt]
                       & \multicolumn{1}{c}{M1} & \multicolumn{1}{c}{M2}         & \multicolumn{1}{c}{M3}         & \multicolumn{1}{c}{M4} & \multicolumn{1}{c}{M5}      & \multicolumn{1}{c}{M6}    & \multicolumn{1}{c}{M7} & \multicolumn{1}{c}{M8} & \multicolumn{1}{c}{M9}    \\ \hline
        tfjs-wasm      & 1.83                   & 1.79                           & 1.61                           & 1.65                   & /                           & /                         & /                      & /                      & /                         \\
        ort.js-wasm    & 1.79                   & 1.49                           & 1.71                           & 1.79                   & 1.66                        & 1.66                      & 4.07                   & 3.71                   & 3.51                      \\
        tfjs-WebGL-I   & 0.77                   & 0.85                           & 1.01                           & 0.82                   & 0.84                        & 0.79                      & 2.10                   & 1.82                   & 1.73                      \\
        tfjs-WebGL-D   & 1.29                   & 1.18                           & 1.51                           & 1.71                   & 1.26                        & 1.49                      & 2.44                   & 3.19                   & 2.85                      \\
        ort.js-WebGL-I & 1.11                   & 1.11                           & 1.31                           & /                      & /                           & /                         & /                      & /                      & /                         \\
        ort.js-WebDL-D & 1.39                   & 1.08                           & 1.14                           & /                      & /                           & /                         & /                      & /                      & /                         \\ \bottomrule[1.5pt]
        \end{tabular}%

    
\end{table*}

==> tex/tab-webgpu.tex <==
\begin{table}[]
    % \linespread{0.75}
    \centering
    \begin{tabular}{@{}ll|rr@{}}
    \toprule[1.5pt]
    \multicolumn{2}{l|}{}               & MobileNetV2 & Resnet50 \\ \midrule
    \multirow{3}{*}{D-GPU} & setup      & 55.8        & 314.5    \\
                           & warming up & 38.0        & 142.1    \\
                           & inference  & 8.7         & 12.4     \\ \midrule
    \multirow{3}{*}{I-GPU} & setup      & 96.1        & 628.3    \\
                           & warming up & 37.3        & 258.3    \\
                           & inference  & 11.2        & 14.5     \\ \bottomrule[1.5pt]
    \end{tabular}
    \caption{End-to-end inference latency (ms) of tf.js in WebGPU backend. ``D-/I-'' indicates discrete/integrated GPU.}
    \label{tab:webgpu}
    \vspace{-4mm}
\end{table}
